Time Series Network Utilization KPI Forecasting Using Advanced AI/ML Models

The rapid proliferation of data-intensive applications, cloud infrastructure, and IoT ecosystems has made proactive resource provisioning critical for maintaining optimal network performance. However, network administrators face a constant battle against capacity constraints, where traditional reactive approaches fail to accurately anticipate traffic fluctuations. This inability to foresee demand leads to costly over-provisioning, unexpected downtime, and degraded quality of service directly impacting operational budgets and business continuity. To achieve efficient capacity planning, accurate forecasting of bandwidth utilization is essential. This study addresses the challenge by evaluating a diverse spectrum of models including seasonal decomposition, Prophet, Random Forest, XGBoost, Support Vector Regression, and advanced deep learning architectures like bidirectional and Convolutional LSTMs - using a common interface dataset benchmarked across MAPE, NRMSE, and R-square metrics. Ultimately, this research delivers actionable insights into the trade-offs between model accuracy and computational efficiency, empowering engineers, operators, and business owners to select the optimal forecasting model for their specific infrastructure needs.

==> figures/new_abstract <==
The findings of this study provide valuable insights into network bandwidth prediction, while also highlighting clear opportunities for future exploration.

To maintain computational efficiency and minimize operational costs—a key priority for lightweight deployments—this research deliberately focused on traditional AI/ML models with low resource requirements, rather than resource-intensive Large Language Models (LLMs) or generative architectures~\cite{ref32}. While the dataset provided a consistent baseline from a single network environment, it naturally established a foundation that future multi-network studies can build upon to capture broader operational variability~\cite{ref33}. Furthermore, the dataset's standard distribution offered a clear view of typical network patterns, leaving the analysis of extreme, high-outlier surge events as an intriguing target for specialized stress-testing studies~\cite{ref31}. Future work could also build on these univariate insights by incorporating multivariate relationships across diverse network parameters~\cite{ref34}.

Looking ahead, expanding this research through adaptive ensemble techniques—fusing diverse model types—presents a strong strategy to further boost prediction robustness and precision~\cite{ref11}. Additionally, while initial model training parameters were intentionally capped to align with the constraints of standard test server environments~\cite{ref08}, scaling these experiments across high-performance computing resources will unlock deeper fine-tuning, extended convergence cycles, and an even more comprehensive evaluation of model reliability~\cite{ref08}.
